Deep Intellectual Property Protection: A Survey

Deep Neural Networks (DNNs), from AlexNet to ResNet to ChatGPT, have made revolutionary progress in recent years, and are widely used in various fields. The high performance of DNNs requires a huge amount of high-quality data, expensive computing hardware, and excellent DNN architectures that are costly to obtain. Therefore, trained DNNs are becoming valuable assets and must be considered the Intellectual Property (IP) of the legitimate owner who created them, in order to protect trained DNN models from illegal reproduction, stealing, redistribution, or abuse. Although being a new emerging and interdisciplinary field, numerous DNN model IP protection methods have been proposed. Given this period of rapid evolution, the goal of this paper is to provide a comprehensive survey of two mainstream DNN IP protection methods: deep watermarking and deep fingerprinting, with a proposed taxonomy. More than 190 research contributions are included in this survey, covering many aspects of Deep IP Protection: problem definition, main threats and challenges, merits and demerits of deep watermarking and deep fingerprinting methods, evaluation metrics, and performance discussion. We finish the survey by identifying promising directions for future research.

==> figure/deepip <==
@inproceedings{white_uchida2017embedding,
  title={Embedding watermarks into deep neural networks},
  author={Uchida, Yusuke and Nagai, Yuki and Sakazawa, Shigeyuki and Satoh, Shin'ichi},
  booktitle={Proceedings of the 2017 ACM on International Conference on Multimedia Retrieval (ICMR)},
  pages={269--277},
  year={2017}
}
@article{white_chen2018deepmarks,
  title={Deepmarks: A digital fingerprinting framework for deep neural networks},
  author={Chen, Huili and Rohani, Bita Darvish and Koushanfar, Farinaz},
  journal={arXiv preprint arXiv:1804.03648},
  year={2018}
}
@inproceedings{bansal2022certified,
  title={Certified Neural Network Watermarks with Randomized Smoothing},
  author={Bansal, Arpit and Chiang, Ping-Yeh and Curry, Michael J and Jain, Rajiv and Wigington, Curtis and Manjunatha, Varun and Dickerson, John P and Goldstein, Tom},
  booktitle={International Conference on Machine Learning},
  pages={1450--1465},
  year={2022},
  organization={PMLR}
}
@inproceedings{white_rouhani2019deepsigns,
  title={Deepsigns: an end-to-end watermarking framework for protecting the ownership of deep neural networks},
  author={Rouhani, Bita Darvish and Chen, Huili and Koushanfar, Farinaz},
  booktitle={ACM International Conference on Architectural Support for Programming Languages and Operating Systems (ASPLOS)},
  year={2019}
}
@article{large_ramesh2022hierarchical,
  title={Hierarchical text-conditional image generation with clip latents},
  author={Ramesh, Aditya and Dhariwal, Prafulla and Nichol, Alex and Chu, Casey and Chen, Mark},
  journal={arXiv preprint arXiv:2204.06125},
  year={2022}
}
@misc{large_openai2023gpt4,
      title={GPT-4 Technical Report}, 
      author={OpenAI},
      year={2023},
      eprint={2303.08774},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}
@inproceedings{wang2019neural,
  title={Neural cleanse: Identifying and mitigating backdoor attacks in neural networks},
  author={Wang, Bolun and Yao, Yuanshun and Shan, Shawn and Li, Huiying and Viswanath, Bimal and Zheng, Haitao and Zhao, Ben Y},
  booktitle={2019 IEEE Symposium on Security and Privacy (SP)},
  pages={707--723},
  year={2019},
  organization={IEEE}
}

@inproceedings{white_feng2020watermarking,
  title={Watermarking neural network with compensation mechanism},
  author={Feng, Le and Zhang, Xinpeng},
  booktitle={International Conference on Knowledge Science, Engineering and Management},
  pages={363--375},
  year={2020},
  organization={Springer}
}
@inproceedings{white_wang2021riga,
  title={Riga: Covert and robust white-box watermarking of deep neural networks},
  author={Wang, Tianhao and Kerschbaum, Florian},
  booktitle={Proceedings of the Web Conference 2021},
  pages={993--1004},
  year={2021}
}
@inproceedings{white_kuribayashi2021white,
  title={White-Box Watermarking Scheme for Fully-Connected Layers in Fine-Tuning Model},
  author={Kuribayashi, Minoru and Tanaka, Takuro and Suzuki, Shunta and Yasui, Tatsuya and Funabiki, Nobuo},
  booktitle={Proceedings of the 2021 ACM Workshop on Information Hiding and Multimedia Security (IH&MMSec)},
  pages={165--170},
  year={2021}
}
@inproceedings{attack_tramer2016stealing,
  title={Stealing machine learning models via prediction $\{$APIs$\}$},
  author={Tram{\`e}r, Florian and Zhang, Fan and Juels, Ari and Reiter, Michael K and Ristenpart, Thomas},
  booktitle={25th USENIX security symposium (USENIX Security 16)},
  pages={601--618},
  year={2016}
}
@inproceedings{attack_wallace2020imitation,
  title={Imitation Attacks and Defenses for Black-box Machine Translation Systems},
  author={Wallace, Eric and Stern, Mitchell and Song, Dawn},
  booktitle={Proceedings of the 2020 Conference on Empirical Methods in Natural Language Processing (EMNLP)},
  pages={5531--5546},
  year={2020}
}
@inproceedings{attack_krishna2019thieves,
  title={Thieves on sesame street! model extraction of bert-based apis},
  author={Krishna, Kalpesh and Tomar, Gaurav Singh and Parikh, Ankur P and Papernot, Nicolas and Iyyer, Mohit},
  journal={ICLR},
  year={2020}
}
@inproceedings{attack_he2021acl,
  title={Model Extraction and Adversarial Transferability, Your BERT is Vulnerable!},
  author={He, Xuanli and Lyu, Lingjuan and Sun, Lichao and Xu, Qiongkai},
  booktitle={Proceedings of the 2021 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies},
  pages={2006--2012},
  year={2021}
}
@inproceedings{white_zhao2021structural,
  title={Structural Watermarking to Deep Neural Networks via Network Channel Pruning},
  author={Zhao, Xiangyu and Yao, Yinzhe and Wu, Hanzhou and Zhang, Xinpeng},
  booktitle={2021 IEEE International Workshop on Information Forensics and Security (WIFS)},
  pages={1--6},
  year={2021},
  organization={IEEE}
}

@article{passport_fan2019rethinking,
  title={Rethinking deep neural network ownership verification: Embedding passports to defeat ambiguity attacks},
  author={Fan, Lixin and Ng, Kam Woh and Chan, Chee Seng},
  journal={Advances in Neural Information Processing Systems},
  volume={32},
  year={2019}
}

@article{passport_fan2021deepip,
  title={DeepIPR: Deep neural network intellectual property protection with passports},
  author={Fan, Lixin and Ng, Kam Woh and Chan, Chee Seng and Yang, Qiang},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  year={2021},
  publisher={IEEE}
}

@article{li2022knowledge,
  title={Knowledge-Free Black-Box Watermark and Ownership Proof for Image Classification Neural Networks},
  author={Li, Fangqi and Wang, Shilin},
  journal={arXiv preprint arXiv:2204.04522},
  year={2022}
}

@article{passport_zhang2020passport,
  title={Passport-aware normalization for deep model protection},
  author={Zhang, Jie and Chen, Dongdong and Liao, Jing and Zhang, Weiming and Hua, Gang and Yu, Nenghai},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={22619--22628},
  year={2020}
}

@article{white_lv2021hufunet,
  title={HufuNet: Embedding the Left Piece as Watermark and Keeping the Right Piece for Ownership Verification in Deep Neural Networks},
  author={Lv, Peizhuo and Li, Pan and Zhang, Shengzhi and Chen, Kai and Liang, Ruigang and Zhao, Yue and Li, Yingjiu},
  journal={arXiv preprint arXiv:2103.13628},
  year={2021}
}


@inproceedings{black_adi2018turning,
  title={Turning your weakness into a strength: Watermarking deep neural networks by backdooring},
  author={Adi, Yossi and Baum, Carsten and Cisse, Moustapha and Pinkas, Benny and Keshet, Joseph},
  booktitle={27th USENIX Security Symposium (USENIX Security 18)},
  pages={1615--1631},
  year={2018}
}

@inproceedings{black_namba2019robust,
  title={Robust watermarking of neural network with exponential weighting},
  author={Namba, Ryota and Sakuma, Jun},
  booktitle={Proceedings of the 2019 ACM Asia Conference on Computer and Communications Security},
  pages={228--240},
  year={2019}
}

@article{black_le2020adversarial,
  title={Adversarial frontier stitching for remote neural network watermarking},
  author={Le Merrer, Erwan and Perez, Patrick and Tr{\'e}dan, Gilles},
  journal={Neural Computing and Applications},
  volume={32},
  number={13},
  pages={9233--9244},
  year={2020},
  publisher={Springer}
}

@inproceedings{black_zhang2018protecting,
  title={Protecting intellectual property of deep neural networks with watermarking},
  author={Zhang, Jialong and Gu, Zhongshu and Jang, Jiyong and Wu, Hui and Stoecklin, Marc Ph and Huang, Heqing and Molloy, Ian},
  booktitle={Proceedings of the 2018 on Asia Conference on Computer and Communications Security},
  pages={159--172},
  year={2018}
}

@inproceedings{black_guo2018watermarking,
  title={Watermarking deep neural networks for embedded systems},
  author={Guo, Jia and Potkonjak, Miodrag},
  booktitle={2018 IEEE/ACM International Conference on Computer-Aided Design (ICCAD)},
  pages={1--8},
  year={2018},
  organization={IEEE}
}

@inproceedings{black_li2019prove,
  title={How to prove your model belongs to you: A blind-watermark based framework to protect intellectual property of DNN},
  author={Li, Zheng and Hu, Chengyu and Zhang, Yang and Guo, Shanqing},
  booktitle={Proceedings of the 35th Annual Computer Security Applications Conference},
  pages={126--137},
  year={2019}
}

@inproceedings{black_zhong2020protecting,
  title={Protecting IP of deep neural networks with watermarking: A new label helps},
  author={Zhong, Qi and Zhang, Leo Yu and Zhang, Jun and Gao, Longxiang and Xiang, Yong},
  booktitle={Pacific-Asia Conference on Knowledge Discovery and Data Mining},
  pages={462--474},
  year={2020},
  organization={Springer}
}

@inproceedings{black_li2020protecting,
  title={Protecting the intellectual property of deep neural networks with watermarking: The frequency domain approach},
  author={Li, Meng and Zhong, Qi and Zhang, Leo Yu and Du, Yajuan and Zhang, Jun and Xiangt, Yong},
  booktitle={2020 IEEE 19th International Conference on Trust, Security and Privacy in Computing and Communications (TrustCom)},
  pages={402--409},
  year={2020},
  organization={IEEE}
}

@article{black_jebreel2021keynet,
  title={Keynet: An asymmetric key-style framework for watermarking deep learning models},
  author={Jebreel, Najeeb Moharram and Domingo-Ferrer, Josep and S{\'a}nchez, David and Blanco-Justicia, Alberto},
  journal={Applied Sciences},
  volume={11},
  number={3},
  pages={999},
  year={2021},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@article{black_sun2021protecting,
  title={Protecting the Intellectual Properties of Deep Neural Networks with an Additional Class and Steganographic Images},
  author={Sun, Shichang and Xue, Mingfu and Wang, Jian and Liu, Weiqiang},
  journal={arXiv preprint arXiv:2104.09203},
  year={2021}
}

@inproceedings{black_szyller2021dawn,
  title={Dawn: Dynamic adversarial watermarking of neural networks},
  author={Szyller, Sebastian and Atli, Buse Gul and Marchal, Samuel and Asokan, N},
  booktitle={Proceedings of the 29th ACM International Conference on Multimedia},
  pages={4417--4425},
  year={2021}
}

@article{black_zhu2020secure,
  title={Secure neural network watermarking protocol against forging attack},
  author={Zhu, Renjie and Zhang, Xinpeng and Shi, Mengte and Tang, Zhenjun},
  journal={EURASIP Journal on Image and Video Processing},
  volume={2020},
  number={1},
  pages={1--12},
  year={2020},
  publisher={Springer}
}

@article{black_li2019piracy,
  title={Piracy resistant watermarks for deep neural networks},
  author={Li, Huiying and Wenger, Emily and Shan, Shawn and Zhao, Ben Y and Zheng, Haitao},
  journal={arXiv preprint arXiv:1910.01226},
  year={2019}
}

@inproceedings{black_maung2021piracy,
  title={Piracy-resistant DNN watermarking by block-wise image transformation with secret key},
  author={Maung Maung, April Pyone and Kiya, Hitoshi},
  booktitle={Proceedings of the 2021 ACM Workshop on Information Hiding and Multimedia Security},
  pages={159--164},
  year={2021}
}

@article{black_aprilpyone2021block,
  title={Block-wise image transformation with secret key for adversarially robust defense},
  author={AprilPyone, MaungMaung and Kiya, Hitoshi},
  journal={IEEE Transactions on Information Forensics and Security},
  volume={16},
  pages={2709--2723},
  year={2021},
  publisher={IEEE}
}

@inproceedings{chen2019deepattest_delete,
  title={Deepattest: an end-to-end attestation framework for deep neural networks},
  author={Chen, Huili and Fu, Cheng and Rouhani, Bita Darvish and Zhao, Jishen and Koushanfar, Farinaz},
  booktitle={2019 ACM/IEEE 46th Annual International Symposium on Computer Architecture (ISCA)},
  pages={487--498},
  year={2019},
  organization={IEEE}
}

@article{black_quan2020watermarking,
  title={Watermarking deep neural networks in image processing},
  author={Quan, Yuhui and Teng, Huan and Chen, Yixin and Ji, Hui},
  journal={IEEE transactions on neural networks and learning systems},
  volume={32},
  number={5},
  pages={1852--1865},
  year={2020},
  publisher={IEEE}
}

@article{esteva2017dermatologist,
	title={Dermatologist level classification of skin cancer with deep neural networks},
	author={Esteva, Andre and Kuprel, Brett and Novoa, Roberto A and Ko, Justin and Swetter, Susan M and Blau, Helen M and Thrun, Sebastian},
	journal={Nature},
	volume={542},
	number={7639},
	pages={115--118},
	year={2017},
	publisher={Nature Publishing Group}
}


@article{hinton2012deep,
  title={Deep neural networks for acoustic modeling in speech recognition: The shared views of four research groups},
  author={Hinton, Geoffrey and Deng, Li and Yu, Dong and Dahl, George E and Mohamed, Abdel-rahman and Jaitly, Navdeep and Senior, Andrew and Vanhoucke, Vincent and Nguyen, Patrick and Sainath, Tara N and others},
  journal={IEEE Signal processing magazine},
  volume={29},
  number={6},
  pages={82--97},
  year={2012},
  publisher={IEEE}
}

@article{devries2018deep,
  title={Deep learning of aftershock patterns following large earthquakes},
  author={DeVries, Phoebe MR and Vi{\'e}gas, Fernanda and Wattenberg, Martin and Meade, Brendan J},
  journal={Nature},
  volume={560},
  number={7720},
  pages={632--634},
  year={2018},
  publisher={Nature Publishing Group}
}

@article{stokes2020deep,
  title={A deep learning approach to antibiotic discovery},
  author={Stokes, Jonathan M and Yang, Kevin and Swanson, Kyle and Jin, Wengong and Cubillos-Ruiz, Andres and Donghia, Nina M and MacNair, Craig R and French, Shawn and Carfrae, Lindsey A and Bloom-Ackerman, Zohar and others},
  journal={Cell},
  volume={180},
  number={4},
  pages={688--702},
  year={2020},
  publisher={Elsevier}
}

@article{silver2018general,
	title={A general reinforcement learning algorithm that masters chess, shogi, and Go through self-play},
	author={Silver, David and Hubert, Thomas and Schrittwieser, Julian and Antonoglou, Ioannis and Lai, Matthew and Guez, Arthur and Lanctot, Marc and Sifre, Laurent and Kumaran, Dharshan and Graepel, Thore and others},
	journal={Science},
	volume={362},
	number={6419},
	pages={1140--1144},
	year={2018},
	publisher={American Association for the Advancement of Science}
}

@article{vinyals2019grandmaster,
	title={Grandmaster level in StarCraft II using multiagent reinforcement learning},
	author={Vinyals, Oriol and Babuschkin, Igor and Czarnecki, Wojciech M and Mathieu, Micha{\"e}l and Dudzik, Andrew and Chung, Junyoung and Choi, David H and Powell, Richard and Ewalds, Timo and Georgiev, Petko and others},
	journal={Nature},
	volume={575},
	number={7782},
	pages={350--354},
	year={2019},
	publisher={Nature Publishing Group}
}


@inproceedings{blace_yadollahi2021robust,
  title={Robust black-box watermarking for deep neural network using inverse document frequency},
  author={Yadollahi, Mohammad Mehdi and Shoeleh, Farzaneh and Dadkhah, Sajjad and Ghorbani, Ali A},
  booktitle={2021 IEEE Intl Conf on Dependable, Autonomic and Secure Computing, Intl Conf on Pervasive Intelligence and Computing, Intl Conf on Cloud and Big Data Computing, Intl Conf on Cyber Science and Technology Congress (DASC/PiCom/CBDCom/CyberSciTech)},
  pages={574--581},
  year={2021},
  organization={IEEE}
}

@article{gray_lou2021meets,
  title={When NAS meets watermarking: ownership verification of DNN models via cache side channels},
  author={Lou, Xiaoxuan and Guo, Shangwei and Zhang, Tianwei and Zhang, Yinqian and Liu, Yang},
  journal={arXiv preprint arXiv:2102.03523},
  year={2021}
}

@article{black_chen2019blackmarks,
  title={Blackmarks: Blackbox multibit watermarking for deep neural networks},
  author={Chen, Huili and Rouhani, Bita Darvish and Koushanfar, Farinaz},
  journal={arXiv preprint arXiv:1904.00344},
  year={2019}
}

@inproceedings{black_jia2021entangled,
  title={Entangled watermarks as a defense against model extraction},
  author={Jia, Hengrui and Choquette-Choo, Christopher A and Chandrasekaran, Varun and Papernot, Nicolas},
  booktitle={30th USENIX Security Symposium (USENIX Security 21)},
  pages={1937--1954},
  year={2021}
}

@inproceedings{black_yang2021robust,
  title={Robust watermarking for deep neural networks via bi-level optimization},
  author={Yang, Peng and Lao, Yingjie and Li, Ping},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={14841--14850},
  year={2021}
}

@inproceedings{attack_chen2021refit,
  title={Refit: a unified watermark removal framework for deep learning systems with limited data},
  author={Chen, Xinyun and Wang, Wenxiao and Bender, Chris and Ding, Yiming and Jia, Ruoxi and Li, Bo and Song, Dawn},
  booktitle={Proceedings of the 2021 ACM Asia Conference on Computer and Communications Security},
  pages={321--335},
  year={2021}
}

@inproceedings{attack_chen2019leveraging,
  title={Leveraging unlabeled data for watermark removal of deep neural networks},
  author={Chen, Xinyun and Wang, Wenxiao and Ding, Yiming and Bender, Chris and Jia, Ruoxi and Li, Bo and Song, Dawn},
  booktitle={ICML workshop on Security and Privacy of Machine Learning},
  pages={1--6},
  year={2019}
}

@inproceedings{attack_wang2019attacks,
  title={Attacks on digital watermarks for deep neural networks},
  author={Wang, Tianhao and Kerschbaum, Florian},
  booktitle={ICASSP 2019-2019 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={2622--2626},
  year={2019},
  organization={IEEE}
}

@article{attack_wang2021detect,
  title={Detect and remove watermark in deep neural networks via generative adversarial networks},
  author={Wang, Haoqi and Xue, Mingfu and Sun, Shichang and Zhang, Yushu and Wang, Jian and Liu, Weiqiang},
  journal={arXiv preprint arXiv:2106.08104},
  year={2021}
}

@article{sok_lukas2021sok,
  title={Sok: How robust is image classification deep neural network watermarking?},
  author={Lukas, Nils and Jiang, Edward and Li, Xinda and Kerschbaum, Florian},
  journal={IEEE S\&P},
  year={2022}
}
@article{survey_oliynyk2022summer,
  title={I Know What You Trained Last Summer: A Survey on Stealing Machine Learning Models and Defences},
  author={Oliynyk, Daryna and Mayer, Rudolf and Rauber, Andreas},
  journal={arXiv preprint arXiv:2206.08451},
  year={2022}
}
@article{attack_chen2022linkbreaker,
  title={LinkBreaker: Breaking the Backdoor-Trigger Link in DNNs via Neurons Consistency Check},
  author={Chen, Zhenzhu and Wang, Shang and Fu, Anmin and Gao, Yansong and Yu, Shui and Deng, Robert H},
  journal={IEEE Transactions on Information Forensics and Security},
  year={2022},
  publisher={IEEE}
}

@article{attack_grosse2020backdoor,
  title={Backdoor Smoothing: Demystifying Backdoor Attacks on Deep Neural Networks},
  author={Grosse, Kathrin and Lee, Taesung and Biggio, Battista and Park, Youngja and Backes, Michael and Molloy, Ian},
  journal={arXiv preprint arXiv:2006.06721},
  year={2020}
}

@article{lou2021novel,
  title={A Novel Watermarking Framework for Ownership Verification of DNN Architectures},
  author={Lou, Xiaoxuan and Guo, Shangwei and Zhang, Tianwei and Li, Jiwei and Zhang, Yinqian and Liu, Yang},
  year={2021}
}

@article{lottery_chen2021you,
  title={You are caught stealing my winning lottery ticket! Making a lottery ticket claim its ownership},
  author={Chen, Xuxi and Chen, Tianlong and Zhang, Zhenyu and Wang, Zhangyang},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={1780--1791},
  year={2021}
} 

@inproceedings{sofiane2021yes,
  title={Yes We can: Watermarking machine learning models beyond classification},
  author={Sofiane, Lounici and Njeh, Mohamed and Ermis, Orhan and {\"O}nen, Melek and Trabelsi, Slim},
  booktitle={CFS 2021, 34th IEEE Computer Security Foundations Symposium},
  year={2021}
}

@inproceedings{fernandez2022watermarking,
  title={Watermarking images in self-supervised latent spaces},
  author={Fernandez, Pierre and Sablayrolles, Alexandre and Furon, Teddy and J{\'e}gou, Herv{\'e} and Douze, Matthijs},
  booktitle={ICASSP 2022-2022 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={3054--3058},
  year={2022},
  organization={IEEE}
}

@article{cong2022sslguard,
  title={SSLGuard: A Watermarking Scheme for Self-supervised Learning Pre-trained Encoders},
  author={Cong, Tianshuo and He, Xinlei and Zhang, Yang},
  journal={arXiv preprint arXiv:2201.11692},
  year={2022}
}

@article{dziedzic2022difficulty,
  title={On the Difficulty of Defending Self-Supervised Learning against Model Extraction},
  author={Dziedzic, Adam and Dhawan, Nikita and Kaleem, Muhammad Ahmad and Guan, Jonas and Papernot, Nicolas},
  journal={arXiv preprint arXiv:2205.07890},
  year={2022}
}

@inproceedings{ong2021protecting,
  title={Protecting intellectual property of generative adversarial networks from ambiguity attacks},
  author={Ong, Ding Sheng and Chan, Chee Seng and Ng, Kam Woh and Fan, Lixin and Yang, Qiang},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={3630--3639},
  year={2021}
}

@article{zhang2021exploring,
  title={Exploring Structure Consistency for Deep Model Watermarking},
  author={Zhang, Jie and Chen, Dongdong and Liao, Jing and Fang, Han and Ma, Zehua and Zhang, Weiming and Hua, Gang and Yu, Nenghai},
  journal={arXiv preprint arXiv:2108.02360},
  year={2021}
}

@article{tang2020deep,
  title={Deep Serial Number: Computational Watermarking for DNN Intellectual Property Protection},
  author={Tang, Ruixiang and Du, Mengnan and Hu, Xia},
  journal={arXiv preprint arXiv:2011.08960},
  year={2020}
}

@article{fan2021fedipr,
  title={FedIPR: Ownership Verification for Federated Deep Neural Network Models},
  author={Fan, Lixin and Li, Bowen and Gu, Hanlin and Li, Jie and Yang, Qiang},
  journal={arXiv preprint arXiv:2109.13236},
  year={2021}
}


@article{alam2022nn,
  title={NN-Lock: A Lightweight Authorization to Prevent IP Threats of Deep Learning Models},
  author={Alam, Manaar and Saha, Sayandeep and Mukhopadhyay, Debdeep and Kundu, Sandip},
  journal={ACM Journal on Emerging Technologies in Computing Systems (JETC)},
  volume={18},
  number={3},
  pages={1--19},
  year={2022},
  publisher={ACM New York, NY}
}

@article{xue2021activeguard,
  title={ActiveGuard: An Active DNN IP Protection Technique via Adversarial Examples},
  author={Xue, Mingfu and Sun, Shichang and He, Can and Zhang, Yushu and Wang, Jian and Liu, Weiqiang},
  journal={arXiv preprint arXiv:2103.01527},
  year={2021}
}

@inproceedings{ito2021access,
  title={Access control using spatially invariant permutation of feature maps for semantic segmentation models},
  author={Ito, Hiroki and AprilPyone, MaungMaung and Kiya, Hitoshi},
  booktitle={2021 Asia-Pacific Signal and Information Processing Association Annual Summit and Conference (APSIPA ASC)},
  pages={1833--1838},
  year={2021},
  organization={IEEE}
}

@article{maungmaung2021protection,
  title={A protection method of trained CNN model with a secret key from unauthorized access},
  author={MaungMaung, AprilPyone and Kiya, Hitoshi},
  journal={APSIPA Transactions on Signal and Information Processing},
  volume={10},
  year={2021},
  publisher={Cambridge University Press}
}

@article{xue2021advparams,
  title={AdvParams: An Active DNN Intellectual Property Protection Technique via Adversarial Perturbation Based Parameter Encryption},
  author={Xue, Mingfu and Wu, Zhiyu and Wang, Jian and Zhang, Yushu and Liu, Weiqiang},
  journal={arXiv preprint arXiv:2105.13697},
  year={2021}
}

@inproceedings{nagamori2022access,
  title={Access Control of Object Detection Models Using Encrypted Feature Maps},
  author={Nagamori, Teru and Ito, Hiroki and AprilPyone, MaungMaung and Kiya, Hitoshi},
  booktitle={2022 IEEE 4th Global Conference on Life Sciences and Technologies (LifeTech)},
  pages={175--178},
  year={2022},
  organization={IEEE}
}

@article{pagnotta2022tattooed,
  title={TATTOOED: A Robust Deep Neural Network Watermarking Scheme based on Spread-Spectrum Channel Coding},
  author={Pagnotta, Giulio and Hitaj, Dorjan and Hitaj, Briland and Perez-Cruz, Fernando and Mancini, Luigi V},
  journal={arXiv preprint arXiv:2202.06091},
  year={2022}
}

@article{none_zhang2021deep,
  title={Deep model intellectual property protection via deep watermarking},
  author={Zhang, Jie and Chen, Dongdong and Liao, Jing and Zhang, Weiming and Feng, Huamin and Hua, Gang and Yu, Nenghai},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  year={2021},
  publisher={IEEE}
}

@article{none_wu2020watermarking,
  title={Watermarking neural networks with watermarked images},
  author={Wu, Hanzhou and Liu, Gen and Yao, Yuwei and Zhang, Xinpeng},
  journal={IEEE Transactions on Circuits and Systems for Video Technology},
  volume={31},
  number={7},
  pages={2591--2601},
  year={2020},
  publisher={IEEE}
}

@inproceedings{aprilpyone2021transfer,
  title={Transfer learning-based model protection with secret key},
  author={AprilPyone, MaungMaung and Kiya, Hitoshi},
  booktitle={2021 IEEE International Conference on Image Processing (ICIP)},
  pages={3877--3881},
  year={2021},
  organization={IEEE}
}


@article{xiang2021protecting,
  title={Protecting Your NLG Models with Semantic and Robust Watermarks},
  author={Xiang, Tao and Xie, Chunlong and Guo, Shangwei and Li, Jiwei and Zhang, Tianwei},
  journal={arXiv preprint arXiv:2112.05428},
  year={2021}
}

@article{passport_lim2022rnn,
  title={Protect, show, attend and tell: Empowering image captioning models with ownership protection},
  author={Lim, Jian Han and Chan, Chee Seng and Ng, Kam Woh and Fan, Lixin and Yang, Qiang},
  journal={Pattern Recognition},
  volume={122},
  pages={108285},
  year={2022},
  publisher={Elsevier}
}

@inproceedings{shafieinejad2021robustness,
  title={On the robustness of backdoor-based watermarking in deep neural networks},
  author={Shafieinejad, Masoumeh and Lukas, Nils and Wang, Jiaqi and Li, Xinda and Kerschbaum, Florian},
  booktitle={Proceedings of the 2021 ACM Workshop on Information Hiding and Multimedia Security},
  pages={177--188},
  year={2021}
}

@inproceedings{white_liu2021watermarking,
  title={Watermarking deep neural networks with greedy residuals},
  author={Liu, Hanwen and Weng, Zhenyu and Zhu, Yuesheng},
  booktitle={International Conference on Machine Learning (ICML)},
  pages={6978--6988},
  year={2021},
  organization={PMLR}
}

@article{li2021regulating,
  title={Regulating ownership verification for deep neural networks: Scenarios, protocols, and prospects},
  author={Li, Fang-Qi and Wang, Shi-Lin and Liew, Alan Wee-Chung},
  journal_={arXiv preprint arXiv:2108.09065},
  journal={IJCAI 2021 Workshop on Toward IPR on Deep Learning as Services}, 
  year={2021}
}

@article{attack_xiang2021peel,
  title={PEEL: A Provable Removal Attack on Deep Hiding},
  author={Xiang, Tao and Liu, Hangcheng and Guo, Shangwei and Zhang, Tianwei},
  journal={arXiv preprint arXiv:2106.02779},
  year={2021}
}

@article{tang2021my,
  title={Was my Model Stolen? Feature Sharing for Robust and Transferable Watermarks},
  author={Tang, Ruixiang and Jin, Hongye and Wigington, Curtis and Du, Mengnan and Jain, Rajiv and Hu, Xia},
  year={2021}
}

@article{zhao2021deep,
  title={Deep Encryption: Protecting Pre-Trained Neural Networks with Confusion Neurons},
  author={Zhao, Mengbiao and Xu, Shixiong and Chang, Jianlong and Xie, Lingxi and Chen, Jie and Tian, Qi},
  year={2021}
}


@inproceedings{iijima2022protection,
  title={Protection of SVM model with secret key from unauthorized access},
  author={Iijima, Ryota and AprilPyone, MaungMaung and Kiay, Hitoshi},
  booktitle={International Workshop on Advanced Imaging Technology (IWAIT) 2022},
  volume={12177},
  pages={509--514},
  year={2022},
  organization={SPIE}
}

@inproceedings{xue2020active,
  title={Active DNN IP protection: a novel user fingerprint management and DNN authorization control technique},
  author={Xue, Mingfu and Wu, Zhiyu and He, Can and Wang, Jian and Liu, Weiqiang},
  booktitle={2020 IEEE 19th International Conference on Trust, Security and Privacy in Computing and Communications (TrustCom)},
  pages={975--982},
  year={2020},
  organization={IEEE}
}

@article{attack_liu2022stolenencoder,
  title={StolenEncoder: Stealing Pre-trained Encoders},
  author={Liu, Yupei and Jia, Jinyuan and Liu, Hongbin and Gong, Neil Zhenqiang},
  journal={arXiv preprint arXiv:2201.05889},
  year={2022}
}

@article{fingerprinting_liu2022your,
  title={Your Model Trains on My Data? Protecting Intellectual Property of Training Data via Membership Fingerprint Authentication},
  author={Liu, Gaoyang and Xu, Tianlong and Ma, Xiaoqiang and Wang, Chen},
  journal={IEEE Transactions on Information Forensics and Security},
  volume={17},
  pages={1024--1037},
  year={2022},
  publisher={IEEE}
}

@inproceedings{fingerprinting_chen2021copy,
  title={Copy, Right? A Testing Framework for Copyright Protection of Deep Learning Models},
  author={Chen, Jialuo and Wang, Jingyi and Peng, Tinglan and Sun, Youcheng and Cheng, Peng and Ji, Shouling and Ma, Xingjun and Li, Bo and Song, Dawn},
  booktitle={IEEE Symposium on Security and Privacy (S\&P)},
  year={2022}
}

@inproceedings{fingerprinting_cao2021ipguard,
  title={IPGuard: Protecting intellectual property of deep neural networks via fingerprinting the classification boundary},
  author={Cao, Xiaoyu and Jia, Jinyuan and Gong, Neil Zhenqiang},
  booktitle={Proceedings of the 2021 ACM Asia Conference on Computer and Communications Security},
  pages={14--25},
  year={2021}
}

@inproceedings{fingerprinting_pan2022metav,
  title={MetaV: A Meta-Verifier Approach to Task-Agnostic Model Fingerprinting},
  author={Pan, Xudong and Yan, Yifan and Zhang, Mi and Yang, Min},
  booktitle={Proceedings of the 28th ACM SIGKDD Conference on Knowledge Discovery and Data Mining},
  pages={1327--1336},
  year={2022}
}

@inproceedings{fingerprinting_wang2021fingerprinting,
  title={Fingerprinting deep neural networks-a deepfool approach},
  author={Wang, Si and Chang, Chip-Hong},
  booktitle={2021 IEEE International Symposium on Circuits and Systems (ISCAS)},
  pages={1--5},
  year={2021},
  organization={IEEE}
}

@article{fingerprinting_li2021novel,
  title={A Novel Verifiable Fingerprinting Scheme for Generative Adversarial Networks},
  author={Li, Guanlin and Xu, Guowen and Qiu, Han and Guo, Shangwei and Wang, Run and Li, Jiwei and Zhang, Tianwei},
  journal={arXiv preprint arXiv:2106.11760},
  year={2021}
}
@inproceedings{fingerprinting_li2021modeldiff,
  title={Modeldiff: testing-based DNN similarity comparison for model reuse detection},
  author={Li, Yuanchun and Zhang, Ziqi and Liu, Bingyan and Yang, Ziyue and Liu, Yunxin},
  booktitle={Proceedings of the 30th ACM SIGSOFT International Symposium on Software Testing and Analysis},
  pages={139--151},
  year={2021}
}
@article{fingerprinting_lukas2019deep,
  title={Deep Neural Network Fingerprinting by Conferrable Adversarial Examples},
  author={Lukas, Nils and Zhang, Yuxuan and Kerschbaum, Florian},
  booktitle={International Conference on Learning Representations},
  year={2020}
}
@inproceedings{fingerprinting_pan2021tafa,
  title={TAFA: A Task-Agnostic Fingerprinting Algorithm for Neural Networks},
  author={Pan, Xudong and Zhang, Mi and Lu, Yifan and Yang, Min},
  booktitle={European Symposium on Research in Computer Security},
  pages={542--562},
  year={2021},
  organization={Springer}
}
@inproceedings{fingerprinting_peng2022fingerprinting,
  title={Fingerprinting Deep Neural Networks Globally via Universal Adversarial Perturbations},
  author={Peng, Zirui and Li, Shaofeng and Chen, Guoxing and Zhang, Cheng and Zhu, Haojin and Xue, Minhui},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={13430--13439},
  year={2022}
}
@article{fingerprinting_zhao2020afa,
  title={AFA: Adversarial fingerprinting authentication for deep neural networks},
  author={Zhao, Jingjing and Hu, Qingyue and Liu, Gaoyang and Ma, Xiaoqiang and Chen, Fei and Hassan, Mohammad Mehedi},
  journal={Computer Communications},
  volume={150},
  pages={488--497},
  year={2020},
  publisher={Elsevier}
}
@inproceedings{none_yu2021artificial,
  title={Artificial fingerprinting for generative models: Rooting deepfake attribution in training data},
  author={Yu, Ning and Skripniuk, Vladislav and Abdelnabi, Sahar and Fritz, Mario},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={14448--14457},
  year={2021}
}
@inproceedings{fingerprinting_wang2021characteristic,
  title={Characteristic Examples: High-Robustness, Low-Transferability Fingerprinting of Neural Networks.},
  author={Wang, Siyue and Wang, Xiao and Chen, Pin-Yu and Zhao, Pu and Lin, Xue},
  booktitle={IJCAI},
  pages={575--582},
  year={2021}
}
@article{fingerprinting_wang2022integrity,
  title={Integrity Fingerprinting of DNN with Double Black-box Design and Verification},
  author={Wang, Shuo and Agarwal, Sidharth and Abuadbba, Sharif and Moore, Kristen and Nepal, Surya and Kanhere, Salil},
  journal={arXiv preprint arXiv:2203.10902},
  year={2022}
}
@article{fingerprinting_dong2021fingerprinting,
  title={Fingerprinting Multi-exit Deep Neural Network Models via Inference Time},
  author={Dong, Tian and Qiu, Han and Zhang, Tianwei and Li, Jiwei and Li, Hewu and Lu, Jialiang},
  journal={arXiv preprint arXiv:2110.03175},
  year={2021}
}


@article{wu2022watermarking,
  title={Watermarking Pre-trained Encoders in Contrastive Learning},
  author={Wu, Yutong and Qiu, Han and Zhang, Tianwei and Qiu, Meikang and others},
  journal={arXiv preprint arXiv:2201.08217},
  year={2022}
}


@inproceedings{hua2021mmguard,
  title={MMGuard: Automatically Protecting On-Device Deep Learning Models in Android Apps},
  author={Hua, Jiayi and Li, Yuanchun and Wang, Haoyu},
  booktitle={2021 IEEE Security and Privacy Workshops (SPW)},
  pages={71--77},
  year={2021},
  organization={IEEE}
}

@inproceedings{fragile_lao2022deepauth,
  title={DeepAuth: A DNN Authentication Framework by Model-Unique and Fragile Signature Embedding},
  author={Lao, Yingjie and Zhao, Weijie and Yang, Peng and Li, Ping},
  booktitle={Proceedings of the Thirty-Sixth AAAI Conference on Artificial Intelligence (AAAI), Virtual Event},
  year={2022}
}

@inproceedings{black_lao2022fewweights,
  title={Identification for Deep Neural Network: Simply Adjusting Few Weights!},
  author={Lao, Yingjie and Yang, Peng and Zhao, Weijie and Li, Ping},
  booktitle={2022 IEEE 38th International Conference on Data Engineering (ICDE)},
  pages={1328--1341},
  year={2022},
  organization={IEEE}
}

@article{zhao2022integrity,
title={Integrity Authentication in Tree Models},
author={Zhao, Weijie and Lao, Yingjie and Li, Ping},
journal={arXiv preprint arXiv:2205.15444},
year={2022}
}

@inproceedings{attack_jagielski2020high,
  title={High accuracy and high fidelity extraction of neural networks},
  author={Jagielski, Matthew and Carlini, Nicholas and Berthelot, David and Kurakin, Alex and Papernot, Nicolas},
  booktitle={29th USENIX security symposium (USENIX Security 20)},
  pages={1345--1362},
  year={2020}
}

@article{devlin2018bert,
  title={{BERT:} Pretraining of deep bidirectional transformers for language understanding},
  author={Devlin, Jacob and Chang, MingWei and Lee, Kenton and Toutanova, Kristina},
  journal={arXiv:1810.04805},
  year={2018}
}


@inproceedings{chen2015deepdriving,
	title={Deepdriving: Learning affordance for direct perception in autonomous driving},
	author={Chen, Chenyi and Seff, Ari and Kornhauser, Alain and Xiao, Jianxiong},
	booktitle={ICCV},
	pages={2722--2730},
	year={2015}
}

@article{Young2018Recent,
  title={Recent trends in deep learning based natural language processing},
  author={Young, Tom and Hazarika, Devamanyu and Poria, Soujanya and Cambria, Erik},
  journal={ieee Computational intelligenCe magazine},
  volume={13},
  number={3},
  pages={55--75},
  year={2018},
  publisher={IEEE}
}

@article{litjens2017survey,
  title={A survey on deep learning in medical image analysis},
  author={Litjens, Geert and Kooi, Thijs and Bejnordi, Babak Ehteshami and Setio, Arnaud Arindra Adiyoso and Ciompi, Francesco and Ghafoorian, Mohsen and Van Der Laak, Jeroen Awm and Van Ginneken, Bram and S{\'a}nchez, Clara I},
  journal={Medical image analysis},
  volume={42},
  pages={60--88},
  year={2017},
  publisher={Elsevier}
}

@article{LeCun15,
  title={Deep learning},
  author={LeCun, Yann and Bengio, Yoshua and Hinton, Geoffrey},
  journal={nature},
  volume={521},
  number={7553},
  pages={436--444},
  year={2015},
  publisher={Nature Publishing Group}
}

@article{pouyanfar2018survey,
  title={A survey on deep learning: Algorithms, techniques, and applications},
  author={Pouyanfar, Samira and Sadiq, Saad and Yan, Yilin and Tian, Haiman and Tao, Yudong and Reyes, Maria Presa and Shyu, Mei-Ling and Chen, Shu-Ching and Iyengar, Sundaraja S},
  journal={ACM Computing Surveys (CSUR)},
  volume={51},
  number={5},
  pages={1--36},
  year={2018},
  publisher={ACM New York, NY, USA}
}

@article{zhu2017deep,
  title={Deep learning in remote sensing: A comprehensive review and list of resources},
  author={Zhu, Xiao Xiang and Tuia, Devis and Mou, Lichao and Xia, Gui-Song and Zhang, Liangpei and Xu, Feng and Fraundorfer, Friedrich},
  journal={IEEE Geoscience and Remote Sensing Magazine},
  volume={5},
  number={4},
  pages={8--36},
  year={2017},
  publisher={IEEE}
}

@article{zhang2018deep,
  title={Deep learning for environmentally robust speech recognition: An overview of recent developments},
  author={Zhang, Zixing and Geiger, J{\"u}rgen and Pohjalainen, Jouni and Mousa, Amr El-Desoky and Jin, Wenyu and Schuller, Bj{\"o}rn},
  journal={ACM Transactions on Intelligent Systems and Technology (TIST)},
  volume={9},
  number={5},
  pages={1--28},
  year={2018},
  publisher={ACM New York, NY, USA}
}

@article{silver2016mastering,
	title={Mastering the game of Go with deep neural networks and tree search},
	author={Silver, David and Huang, Aja and Maddison, Chris J and Guez, Arthur and Sifre, Laurent and Van Den Driessche, George and Schrittwieser, Julian and Antonoglou, Ioannis and Panneershelvam, Veda and Lanctot, Marc and others},
	journal={Nature},
	volume={529},
	number={7587},
	pages={484},
	year={2016},
	publisher={Nature Publishing Group}
}

@article{silver2017mastering,
	title={Mastering the game of go without human knowledge},
	author={Silver, David and Schrittwieser, Julian and Simonyan, Karen and Antonoglou, Ioannis and Huang, Aja and Guez, Arthur and Hubert, Thomas and Baker, Lucas and Lai, Matthew and Bolton, Adrian and others},
	journal={Nature},
	volume={550},
	number={7676},
	pages={354--359},
	year={2017},
	publisher={Nature Publishing Group}
}

@article{brown2019superhuman,
	title={Superhuman AI for multiplayer poker},
	author={Brown, Noam and Sandholm, Tuomas},
	journal={Science},
	volume={365},
	number={6456},
	pages={885--890},
	year={2019},
	publisher={American Association for the Advancement of Science}
}

@inproceedings{taigman2014deepface,
	title={{DeepFace}: Closing the gap to human-level performance in face verification},
	author={Taigman, Yaniv and Yang, Ming and Ranzato, Marc'Aurelio and Wolf, Lior},
	booktitle={CVPR},
	pages={1701--1708},
	year={2014}
}


@article{liu1809deepa,
	title={Deep learning for generic object detection: A survey},
	author={Liu, Li and Ouyang, Wanli and Wang, Xiaogang and Fieguth, Paul and Chen, Jie and Liu, Xinwang and Pietik{\"a}inen, Matti},
	journal={IJCV},
	pages={261-318},
  volume={128},
	year={2020},
  number={2},
	publisher={Springer}
}


@inproceedings{orekondy2019prediction,
  title={Prediction Poisoning: Towards Defenses Against DNN Model Stealing Attacks},
  author={Orekondy, Tribhuvanesh and Schiele, Bernt and Fritz, Mario},
  booktitle={International Conference on Learning Representations},
  year={2019}
}

@inproceedings{krizhevsky2012imagenet,
	title={Imagenet classification with deep convolutional neural networks},
	author={Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E},
	booktitle={NeurIPS},
	pages={1097--1105},
	year={2012}
}



@inproceedings{liu2021removing,
  title={Removing backdoor-based watermarks in neural networks with limited data},
  author={Liu, Xuankai and Li, Fengting and Wen, Bihan and Li, Qi},
  booktitle={2020 25th International Conference on Pattern Recognition (ICPR)},
  pages={10149--10156},
  year={2021},
  organization={IEEE}
}

@inproceedings{zhang2020model,
  title={Model watermarking for image processing networks},
  author={Zhang, Jie and Chen, Dongdong and Liao, Jing and Fang, Han and Zhang, Weiming and Zhou, Wenbo and Cui, Hao and Yu, Nenghai},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={34},
  number={07},
  pages={12805--12812},
  year={2020}
}

@article{goldblum2022dataset,
  title={Dataset security for machine learning: Data poisoning, backdoor attacks, and defenses},
  author={Goldblum, Micah and Tsipras, Dimitris and Xie, Chulin and Chen, Xinyun and Schwarzschild, Avi and Song, Dawn and Madry, Aleksander and Li, Bo and Goldstein, Tom},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  year={2022},
  publisher={IEEE}
}

@article{Bengio13Feature,
  title={Representation Learning: A Review and New Perspectives},
  author={Y. Bengio and A. Courville and P. Vincent},
  journal={IEEE TPAMI},
  volume={35},
  number={8},
  pages={1798--1828},
  year={2013},
language={English}
}

@article{wang2019robust,
  title={Robust and undetectable white-box watermarks for deep neural networks},
  author={Wang, Tianhao and Kerschbaum, Florian},
  journal={arXiv preprint arXiv:1910.14268},
  volume={1},
  number={2},
  year={2019}
}

@book{Goodfellow2016Deep,
  title={Deep Learning},
  author={Goodfellow, Ian and Bengio, Yoshua and Courville, Aaron},
  year={2016},
  publisher={MIT press}
}


@inproceedings{chen2019deepattest,
  title={Deepattest: an end-to-end attestation framework for deep neural networks},
  author={Chen, Huili and Fu, Cheng and Rouhani, Bita Darvish and Zhao, Jishen and Koushanfar, Farinaz},
  booktitle={2019 ACM/IEEE 46th Annual International Symposium on Computer Architecture (ISCA)},
  pages={487--498},
  year={2019},
  organization={IEEE}
}

@inproceedings{chakraborty2020hardware,
  title={Hardware-assisted intellectual property protection of deep learning models},
  author={Chakraborty, Abhishek and Mondai, Ankit and Srivastava, Ankur},
  booktitle={2020 57th ACM/IEEE Design Automation Conference (DAC)},
  pages={1--6},
  year={2020},
  organization={IEEE}
}



@article{yang2019effectiveness,
  title={Effectiveness of distillation attack and countermeasure on neural network watermarking},
  author={Yang, Ziqi and Dang, Hung and Chang, Ee-Chien},
  journal={arXiv preprint arXiv:1906.06046},
  year={2019}
}

@inproceedings{chen2018protect,
  title={Protect your deep neural networks from piracy},
  author={Chen, Mingliang and Wu, Min},
  booktitle={2018 IEEE International Workshop on Information Forensics and Security (WIFS)},
  pages={1--7},
  year={2018},
  organization={IEEE}
}

@inproceedings{sakazawa2019visual,
  title={Visual decoding of hidden watermark in trained deep neural network},
  author={Sakazawa, Shigeyuki and Myodo, Emi and Tasaka, Kazuyuki and Yanagihara, Hiromasa},
  booktitle={2019 IEEE Conference on Multimedia Information Processing and Retrieval (MIPR)},
  pages={371--374},
  year={2019},
  organization={IEEE}
}

@inproceedings{passport_ong2021iprgan,
  title={Protecting intellectual property of generative adversarial networks from ambiguity attacks},
  author={Ong, Ding Sheng and Chan, Chee Seng and Ng, Kam Woh and Fan, Lixin and Yang, Qiang},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition  (CVPR)},
  pages={3630--3639},
  year={2021}
}

@article{lin2020chaotic,
  title={Chaotic weights: A novel approach to protect intellectual property of deep neural networks},
  author={Lin, Ning and Chen, Xiaoming and Lu, Hang and Li, Xiaowei},
  journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems},
  volume={40},
  number={7},
  pages={1327--1339},
  year={2020},
  publisher={IEEE}
}


@inproceedings{guan2020reversible,
  title={Reversible watermarking in deep convolutional neural networks for integrity authentication},
  author={Guan, Xiquan and Feng, Huamin and Zhang, Weiming and Zhou, Hang and Zhang, Jie and Yu, Nenghai},
  booktitle={Proceedings of the 28th ACM International Conference on Multimedia},
  pages={2273--2280},
  year={2020}
}

@inproceedings{pyone2020training,
  title={Training dnn model with secret key for model protection},
  author={Pyone, April and Maung, Maung and Kiya, Hitoshi},
  booktitle={2020 IEEE 9th Global Conference on Consumer Electronics (GCCE)},
  pages={818--821},
  year={2020},
  organization={IEEE}
}

@article{atli2020waffle,
  title={WAFFLE: watermarking in federated learning},
  author={Atli, Buse Gul and Xia, Yuxi and Marchal, Samuel and Asokan, N},
  journal={arXiv preprint arXiv:2008.07298},
  year={2020}
}

@inproceedings{chen2021stealing,
  title={Stealing deep reinforcement learning models for fun and profit},
  author={Chen, Kangjie and Guo, Shangwei and Zhang, Tianwei and Xie, Xiaofei and Liu, Yang},
  booktitle={Proceedings of the 2021 ACM Asia Conference on Computer and Communications Security},
  pages={307--319},
  year={2021}
}

@article{chen2018performance,
  title={Performance comparison of contemporary dnn watermarking techniques},
  author={Chen, Huili and Rouhani, Bita Darvish and Fan, Xinwei and Kilinc, Osman Cihan and Koushanfar, Farinaz},
  journal={arXiv preprint arXiv:1811.03713},
  year={2018}
}

@article{yu2020responsible,
  title={Responsible disclosure of generative models using scalable fingerprinting},
  author={Yu, Ning and Skripniuk, Vladislav and Chen, Dingfan and Davis, Larry and Fritz, Mario},
  journal={arXiv preprint arXiv:2012.08726},
  year={2020}
}

@article{xu2020identity,
  title={“identity bracelets” for deep neural networks},
  author={Xu, Xiangrui and Li, Yaqin and Yuan, Cao},
  journal={IEEE Access},
  volume={8},
  pages={102065--102074},
  year={2020},
  publisher={IEEE}
}

@inproceedings{abdelnabi2021adversarial,
  title={Adversarial watermarking transformer: Towards tracing text provenance with data hiding},
  author={Abdelnabi, Sahar and Fritz, Mario},
  booktitle={2021 IEEE Symposium on Security and Privacy (SP)},
  pages={121--140},
  year={2021},
  organization={IEEE}
}

@inproceedings{chen2019invisible,
  title={Invisible poisoning: Highly stealthy targeted poisoning attack},
  author={Chen, Jinyin and Zheng, Haibin and Su, Mengmeng and Du, Tianyu and Lin, Changting and Ji, Shouling},
  booktitle={International Conference on Information Security and Cryptology},
  pages={173--198},
  year={2019},
  organization={Springer}
}

@inproceedings{ma2021undistillable,
  title={Undistillable: Making a nasty teacher that cannot teach students},
  author={Ma, Haoyu and Chen, Tianlong and Hu, Ting-Kuei and You, Chenyu and Xie, Xiaohui and Wang, Zhangyang},
  journal={ICLR},
  year={2021}
}

@inproceedings{ge2021anti,
  title={Anti-distillation backdoor attacks: Backdoors can really survive in knowledge distillation},
  author={Ge, Yunjie and Wang, Qian and Zheng, Baolin and Zhuang, Xinlu and Li, Qi and Shen, Chao and Wang, Cong},
  booktitle={Proceedings of the 29th ACM International Conference on Multimedia},
  pages={826--834},
  year={2021}
}

@article{ye2021safe,
  title={Safe Distillation Box},
  author={Ye, Jingwen and Mao, Yining and Song, Jie and Wang, Xinchao and Jin, Cheng and Song, Mingli},
  journal={arXiv preprint arXiv:2112.03695},
  year={2021}
}

@article{Wu2019Comprehensive,
  title={A comprehensive survey on graph neural networks},
  author={Wu, Zonghan and Pan, Shirui and Chen, Fengwen and Long, Guodong and Zhang, Chengqi and Philip, S Yu},
  journal={IEEE transactions on neural networks and learning systems},
  volume={32},
  number={1},
  pages={4--24},
  year={2020},
  publisher={IEEE}
}

@article{zhou2020graph,
  title={Graph neural networks: A review of methods and applications},
  author={Zhou, Jie and Cui, Ganqu and Hu, Shengding and Zhang, Zhengyan and Yang, Cheng and Liu, Zhiyuan and Wang, Lifeng and Li, Changcheng and Sun, Maosong},
  journal={AI Open},
  volume={1},
  pages={57--81},
  year={2020},
  publisher={Elsevier}
}

@article{kundu2021analyzing,
  title={Analyzing the confidentiality of undistillable teachers in knowledge distillation},
  author={Kundu, Souvik and Sun, Qirui and Fu, Yao and Pedram, Massoud and Beerel, Peter},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={9181--9192},
  year={2021}
}

@inproceedings{ma2022sparse,
  title={Sparse Logits Suffice to Fail Knowledge Distillation},
  author={Ma, Haoyu and Huang, Yifan and Tang, Hao and You, Chenyu and Kong, Deying and Xie, Xiaohui},
  booktitle={ICLR 2022 Workshop on $PAIR^2$ Struct},
  year={2022}
}

@article{guo2019evolutionary,
  title={Evolutionary trigger set generation for dnn black-box watermarking},
  author={Guo, Jia and Potkonjak, Miodrag},
  journal={arXiv preprint arXiv:1906.04411},
  year={2019}
}

@inproceedings{chen2020specmark,
  title={SpecMark: A Spectral Watermarking Framework for IP Protection of Speech Recognition Systems.},
  author={Chen, Huili and Rouhani, Bita Darvish and Koushanfar, Farinaz},
  booktitle={INTERSPEECH},
  pages={2312--2316},
  year={2020}
}

@inproceedings{chen2021temporal,
  title={Temporal watermarks for deep reinforcement learning models},
  author={Chen, Kangjie and Guo, Shangwei and Zhang, Tianwei and Li, Shuxin and Liu, Yang},
  booktitle={Proceedings of the 20th International Conference on Autonomous Agents and MultiAgent Systems},
  pages={314--322},
  year={2021}
}

@article{li2021spread,
  title={Spread-transform dither modulation watermarking of deep neural network},
  author={Li, Yue and Tondi, Benedetta and Barni, Mauro},
  journal={Journal of Information Security and Applications},
  volume={63},
  pages={103004},
  year={2021},
  publisher={Elsevier}
}

@inproceedings{mosafi2019stealing,
  title={Stealing knowledge from protected deep neural networks using composite unlabeled data},
  author={Mosafi, Itay and David, Eli Omid and Netanyahu, Nathan S},
  booktitle={2019 International Joint Conference on Neural Networks (IJCNN)},
  pages={1--8},
  year={2019},
  organization={IEEE}
}

@article{souri2021sleeper,
  title={Sleeper agent: Scalable hidden trigger backdoors for neural networks trained from scratch},
  author={Souri, Hossein and Goldblum, Micah and Fowl, Liam and Chellappa, Rama and Goldstein, Tom},
  journal={arXiv preprint arXiv:2106.08970},
  year={2021}
}


@article{zhang2020deeptrigger,
  title={DeepTrigger: A watermarking scheme of deep learning models based on chaotic automatic data annotation},
  author={Zhang, Ying-Qian and Jia, Yi-Ran and Wang, Xingyuan and Niu, Qiong and Chen, Nian-Dong},
  journal={IEEE Access},
  volume={8},
  pages={213296--213305},
  year={2020},
  publisher={IEEE}
} 

@inproceedings{zhao2021watermarking,
  title={Watermarking graph neural networks by random graphs},
  author={Zhao, Xiangyu and Wu, Hanzhou and Zhang, Xinpeng},
  booktitle={2021 9th International Symposium on Digital Forensics and Security (ISDFS)},
  pages={1--6},
  year={2021},
  organization={IEEE}
}

@inproceedings{zanella2021grey,
  title={Grey-box extraction of natural language models},
  author={Zanella-Beguelin, Santiago and Tople, Shruti and Paverd, Andrew and K{\"o}pf, Boris},
  booktitle={International Conference on Machine Learning (ICML)},
  pages={12278--12286},
  year={2021},
  organization={PMLR}
}

@article{li2021secure,
  title={Secure watermark for deep neural networks with multi-task learning},
  author={Li, Fangqi and Wang, Shilin},
  journal={arXiv preprint arXiv:2103.10021},
  year={2021}
}

@article{survey_regazzoni2021protecting,
  title={Protecting artificial intelligence IPs: a survey of watermarking and fingerprinting for machine learning},
  author={Regazzoni, Francesco and Palmieri, Paolo and Smailbegovic, Fethulah and Cammarota, Rosario and Polian, Ilia},
  journal={CAAI Transactions on Intelligence Technology},
  volume={6},
  number={2},
  pages={180--191},
  year={2021},
  publisher={Wiley Online Library}
}

@article{survey_boenisch2020survey,
  title={A survey on model watermarking neural networks},
  author={Boenisch, Franziska},
  journal={arXiv preprint arXiv:2009.12153},
  year={2020}
}

@article{survey_xue2022intellectual,
  title={Intellectual Property Protection for Deep Learning Models: Taxonomy, Methods, Attacks, and Evaluations},
  author={Xue, Mingfu and Zhang, Yushu and Wang, Jian and Liu, Weiqiang},
  journal={IEEE Transactions on Artificial Intelligence},
  volume={1},
  number={01},
  pages={1--1},
  year={2022},
  publisher={IEEE Computer Society}
}



@article{guo2020fine,
  title={Fine-tuning is not enough: A simple yet effective watermark removal attack for dnn models},
  author={Guo, Shangwei and Zhang, Tianwei and Qiu, Han and Zeng, Yi and Xiang, Tao and Liu, Yang},
  journal={arXiv preprint arXiv:2009.08697},
  year={2020}
}

@inproceedings{kuribayashi2020deepwatermark,
  title={Deepwatermark: Embedding watermark into DNN model},
  author={Kuribayashi, Minoru and Tanaka, Takuro and Funabiki, Nobuo},
  booktitle={2020 Asia-Pacific Signal and Information Processing Association Annual Summit and Conference (APSIPA ASC)},
  pages={1340--1346},
  year={2020},
  organization={IEEE}
}

@article{sun2020shadownet,
  title={ShadowNet: A secure and efficient system for on-device model inference},
  author={Sun, Zhichuang and Sun, Ruimin and Liu, Changming and Chowdhury, Amrita Roy and Jha, Somesh and Lu, Long},
  journal={arXiv preprint arXiv:2011.05905},
  year={2020}
}

@inproceedings{li2021persistent,
  title={Persistent watermark for image classification neural networks by penetrating the autoencoder},
  author={Li, Fang-Qi and Wang, Shi-Lin},
  booktitle={2021 IEEE International Conference on Image Processing (ICIP)},
  pages={3063--3067},
  year={2021},
  organization={IEEE}
}

@article{xia2020watermarking,
  title={Watermarking federated deep neural network models},
  author={Xia, Yuxi and others},
  year={2020}
}
@article{botta2021neunac,
  title={NeuNAC: A novel fragile watermarking algorithm for integrity protection of neural networks},
  author={Botta, Marco and Cavagnino, Davide and Esposito, Roberto},
  journal={Information Sciences},
  volume={576},
  pages={228--241},
  year={2021},
  publisher={Elsevier}
}

@article{song2019robust,
  title={Robust Membership Encoding: Inference Attacks and Copyright Protection for Deep Learning},
  author={Song, Congzheng and Shokri, Reza},
  journal={arXiv preprint arXiv:1909.12982},
  year={2019}
}

@article{gomez2019security,
  title={Security for Distributed Deep Neural Networks Towards Data Confidentiality \& Intellectual Property Protection},
  author={Gomez, Laurent and Wilhelm, Marcus and M{\'a}rquez, Jos{\'e} and Duverger, Patrick},
  journal={arXiv preprint arXiv:1907.04246},
  year={2019}
}

@inproceedings{tartaglione2021delving,
  title={Delving in the loss landscape to embed robust watermarks into neural networks},
  author={Tartaglione, Enzo and Grangetto, Marco and Cavagnino, Davide and Botta, Marco},
  booktitle={2020 25th International Conference on Pattern Recognition (ICPR)},
  pages={1243--1250},
  year={2021},
  organization={IEEE}
}


@article{wang2022protecting,
  title={Protecting the Intellectual Property of Speaker Recognition Model by Black-Box Watermarking in the Frequency Domain},
  author={Wang, Yumin and Wu, Hanzhou},
  journal={Symmetry},
  volume={14},
  number={3},
  pages={619},
  year={2022},
  publisher={MDPI}
}

@article{li2021towards,
  title={Towards practical watermark for deep neural networks in federated learning},
  author={Li, Fang-Qi and Wang, Shi-Lin and Liew, Alan Wee-Chung},
  journal={arXiv preprint arXiv:2105.03167},
  year={2021}
}

@article{xu2019novel,
  title={A novel method for identifying the deep neural network model with the Serial Number},
  author={Xu, XiangRui and Li, YaQin and Yuan, Cao},
  journal={arXiv preprint arXiv:1911.08053},
  year={2019}
}


@inproceedings{song2020membership,
  title={Membership encoding for deep learning},
  author={Song, Congzheng and Shokri, Reza},
  booktitle={Proceedings of the 15th ACM Asia Conference on Computer and Communications Security},
  pages={344--356},
  year={2020}
}

@inproceedings{barni2021dnn,
  title={DNN watermarking: four challenges and a funeral},
  author={Barni, Mauro and P{\'e}rez-Gonz{\'a}lez, Fernando and Tondi, Benedetta},
  booktitle={Proceedings of the 2021 ACM Workshop on Information Hiding and Multimedia Security},
  pages={189--196},
  year={2021}
}

@inproceedings{nlp_he2022dawnnlp,
  title={Protecting intellectual property of language generation apis with lexical watermark},
  author={He, Xuanli and Xu, Qiongkai and Lyu, Lingjuan and Wu, Fangzhao and Wang, Chenguang},
  year={2022},
  organization={AAAI}
}

@inproceedings{he2021weight,
  title={A weight-wise watermarking technique for DNN models and its robustness against overwriting attack},
  author={He, Han and Kang, Seok and Sakamoto, Yuji},
  booktitle={International Workshop on Advanced Imaging Technology (IWAIT) 2021},
  volume={11766},
  pages={442--446},
  year={2021},
  organization={SPIE}
}

@article{xue2022active,
  title={Active intellectual property protection for deep neural networks through stealthy backdoor and users’ identities authentication},
  author={Xue, Mingfu and Sun, Shichang and Zhang, Yushu and Wang, Jian and Liu, Weiqiang},
  journal={Applied Intelligence},
  pages={1--15},
  year={2022},
  publisher={Springer}
}

@inproceedings{zhu2021fragile,
  title={Fragile Neural Network Watermarking with Trigger Image Set},
  author={Zhu, Renjie and Wei, Ping and Li, Sheng and Yin, Zhaoxia and Zhang, Xinpeng and Qian, Zhenxing},
  booktitle={International Conference on Knowledge Science, Engineering and Management},
  pages={280--293},
  year={2021},
  organization={Springer}
}

@inproceedings{gupta2021digital,
  title={Digital Watermarking to Protect Deep Learning Model},
  author={Gupta, Laveesh and Gupta, Muskan and Khaitan, Nishit and Mundada, Monica R and others},
  booktitle={International Conference on Intelligent and Smart Computing in Data Analytics},
  pages={207--214},
  year={2021},
  organization={Springer}
}

@inproceedings{aprilpyone2021transfer,
  title={Transfer learning-based model protection with secret key},
  author={AprilPyone, MaungMaung and Kiya, Hitoshi},
  booktitle={2021 IEEE International Conference on Image Processing (ICIP)},
  pages={3877--3881},
  year={2021},
  organization={IEEE}
}

@article{wang2021data,
  title={Data Hiding in Neural Networks for Multiple Receivers [Research Frontier]},
  author={Wang, Zichi and Feng, Guorui and Wu, Hanzhou and Zhang, Xinpeng},
  journal={IEEE Computational Intelligence Magazine},
  volume={16},
  number={4},
  pages={70--84},
  year={2021},
  publisher={IEEE}
}

@inproceedings{deeba2019protecting,
  title={Protecting the Intellectual Properties of Digital Watermark Using Deep Neural Network},
  author={Deeba, Farah and Tefera, Getenet and Kun, She and Memon, Hira},
  booktitle={2019 4th International Conference on Information Systems Engineering (ICISE)},
  pages={91--95},
  year={2019},
  organization={IEEE}
}


@inproceedings{li2022encryption,
  title={Encryption Resistant Deep Neural Network Watermarking},
  author={Li, Guobiao and Li, Sheng and Qian, Zhenxing and Zhang, Xinpeng},
  booktitle={ICASSP 2022-2022 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={3064--3068},
  year={2022},
  organization={IEEE}
}

@inproceedings{mehta2022aime,
  title={AIME: watermarking AI models by leveraging errors},
  author={Mehta, Dhwani and Mondol, Nurun and Farahmandi, Farimah and Tehranipoor, Mark},
  booktitle={2022 Design, Automation \& Test in Europe Conference \& Exhibition (DATE)},
  pages={304--309},
  year={2022},
  organization={IEEE}
}

@inproceedings{chattopadhyay2021rowback,
  title={ROWBACK: RObust Watermarking for neural networks using BACKdoors},
  author={Chattopadhyay, Nandish and Chattopadhyay, Anupam},
  booktitle={2021 20th IEEE International Conference on Machine Learning and Applications (ICMLA)},
  pages={1728--1735},
  year={2021},
  organization={IEEE}
}

@inproceedings{he2020parameters,
  title={A Parameters Sharing Watermarking Technique for Convolutional Neural Network Model},
  author={He, Han and Kang, Seok and Sakamoto, Yuji},
  booktitle={Forum on Information Technology},
  year={2020}
}

@incollection{rathi2018revival,
  title={Revival of the Neural Networks and the Intellectual Property Nightmare},
  author={Rathi, Shubham},
  booktitle={Intelligent Environments 2018},
  pages={275--284},
  year={2018},
  publisher={IOS Press}
}

@article{kuribayashi2021immunization,
  title={Immunization of Pruning Attack in DNN Watermarking Using Constant Weight Code},
  author={Kuribayashi, Minoru and Yasui, Tatsuya and Malik, Asad and Funabiki, Nobuo},
  journal={arXiv preprint arXiv:2107.02961},
  year={2021}
}

@inproceedings{li2022fostering,
  title={Fostering The Robustness Of White-Box Deep Neural Network Watermarks By Neuron Alignment},
  author={Li, Fang-Qi and Wang, Shi-Lin and Zhu, Yun},
  booktitle={ICASSP 2022-2022 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={3049--3053},
  year={2022},
  organization={IEEE}
}

@article{survey_li2021nc,
  title={A survey of deep neural network watermarking techniques},
  author={Li, Yue and Wang, Hongxia and Barni, Mauro},
  journal={Neurocomputing},
  volume={461},
  pages={171--193},
  year={2021},
  publisher={Elsevier}
}

@article{survey_boenisch2021systematic,
  title={A systematic review on model watermarking for neural networks},
  author={Boenisch, Franziska},
  journal={Frontiers in big Data},
  volume={4},
  year={2021},
  publisher={Frontiers Media SA}
}

@inproceedings{li2019deepkeystego,
  title={DeepKeyStego: Protecting Communication by Key-dependent Steganography with Deep Networks},
  author={Li, Zheng and Han, Ge and Guo, Shanqing and Hu, Chengyu},
  booktitle={2019 IEEE 21st International Conference on High Performance Computing and Communications; IEEE 17th International Conference on Smart City; IEEE 5th International Conference on Data Science and Systems (HPCC/SmartCity/DSS)},
  pages={1937--1944},
  year={2019},
  organization={IEEE}
}


@inproceedings{yamaji2022tolerance,
  title={Tolerance of CNN watermarking against model optimizations},
  author={Yamaji, Yudai and Sakazawa, Shigeyuki},
  booktitle={International Workshop on Advanced Imaging Technology (IWAIT) 2022},
  volume={12177},
  pages={347--352},
  year={2022},
  organization={SPIE}
}

@inproceedings{vybornova2022method,
  title={Method for copyright protection of deep neural networks using digital watermarking},
  author={Vybornova, Yuliya},
  booktitle={Fourteenth International Conference on Machine Vision (ICMV 2021)},
  volume={12084},
  pages={297--304},
  year={2022},
  organization={SPIE}
}

@inproceedings{black_bansal2022certified,
  title={Certified Neural Network Watermarks with Randomized Smoothing},
  author={Bansal, Arpit and Chiang, Ping-yeh and Curry, Michael J and Jain, Rajiv and Wigington, Curtis and Manjunatha, Varun and Dickerson, John P and Goldstein, Tom},
  booktitle={International Conference on Machine Learning (ICML)},
  pages={1450--1465},
  year={2022},
  organization={PMLR}
}

@article{fkirin2022copyright,
  title={Copyright protection of deep neural network models using digital watermarking: a comparative study},
  author={Fkirin, Alaa and Attiya, Gamal and El-Sayed, Ayman and Shouman, Marwa A},
  journal={Multimedia Tools and Applications},
  volume={81},
  number={11},
  pages={15961--15975},
  year={2022},
  publisher={Springer}
}

@inproceedings{tai2020distributed,
  title={Distributed Watermarking for Cross-Domain of Semantic Large Image Database},
  author={Tai, Le Danh and Thang, Nguyen Kim and Thanh, Ta Minh},
  booktitle={International Conference on Industrial Networks and Intelligent Systems},
  pages={163--180},
  year={2020},
  organization={Springer}
}

@article{lin2022verifying,
  title={Verifying Integrity of Deep Ensemble Models by Lossless Black-box Watermarking with Sensitive Samples},
  author={Lin, Lina and Wu, Hanzhou},
  journal={arXiv preprint arXiv:2205.04145},
  year={2022}
}

@article{gao2022verifi,
  title={VeriFi: Towards Verifiable Federated Unlearning},
  author={Gao, Xiangshan and Ma, Xingjun and Wang, Jingyi and Sun, Youcheng and Li, Bo and Ji, Shouling and Cheng, Peng and Chen, Jiming},
  journal={arXiv preprint arXiv:2205.12709},
  year={2022}
}

@article{wu2021hiding,
  title={Hiding Data Hiding},
  author={Wu, Hanzhou and Liu, Gen and Zhang, Xinpeng},
  journal={arXiv preprint arXiv:2102.06826},
  year={2021}
}

@article{tekgul2022effectiveness,
  title={On the Effectiveness of Dataset Watermarking in Adversarial Settings},
  author={Tekgul, Buse Gul Atli and Asokan, N},
  journal={arXiv preprint arXiv:2202.12506},
  year={2022}
}

@inproceedings{kapusta2021protocol,
  title={A Protocol for Secure Verification of Watermarks Embedded into Machine Learning Models},
  author={Kapusta, Katarzyna and Thouvenot, Vincent and Bettan, Olivier and Beguinet, Hugo and Senet, Hugo},
  booktitle={Proceedings of the 2021 ACM Workshop on Information Hiding and Multimedia Security},
  pages={171--176},
  year={2021}
}

@inproceedings{li2021feature,
  title={A Feature-Map-Based Large-Payload DNN Watermarking Algorithm},
  author={Li, Yue and Abady, Lydia and Wang, Hongxia and Barni, Mauro},
  booktitle={International Workshop on Digital Watermarking},
  pages={135--148},
  year={2021},
  organization={Springer}
}

@inproceedings{wang2021deeptrace,
  title={DeepTrace: A Secure Fingerprinting Framework for Intellectual Property Protection of Deep Neural Networks},
  author={Wang, Runhao and Kang, Jiexiang and Yin, Wei and Wang, Hui and Sun, Haiying and Chen, Xiaohong and Gao, Zhongjie and Wang, Shuning and Liu, Jing},
  booktitle={2021 IEEE 20th International Conference on Trust, Security and Privacy in Computing and Communications (TrustCom)},
  pages={188--195},
  year={2021},
  organization={IEEE}
}

@inproceedings{kakikura2022collusion,
  title={Collusion Resistant Watermarking for Deep Learning Models Protection},
  author={Kakikura, Sayoko and Kang, Hyunho and Iwamura, Keiichi},
  booktitle={2022 24th International Conference on Advanced Communication Technology (ICACT)},
  pages={40--43},
  year={2022},
  organization={IEEE}
}

@article{xue2021protect,
  title={Protect the Intellectual Property of Dataset against Unauthorized Use},
  author={Xue, Mingfu and Wu, Yinghao and Zhang, Yushu and Wang, Jian and Liu, Weiqiang},
  journal={arXiv preprint arXiv:2109.07921},
  year={2021}
}

@article{black_charette2022cosine,
  title={Cosine Model Watermarking Against Ensemble Distillation},
  author={Charette, Laurent and Chu, Lingyang and Chen, Yizhou and Pei, Jian and Wang, Lanjun and Zhang, Yong},
  journal={AAAI 2022},
  year={2022}
}

@article{clements2022deephardmark,
  title={DeepHardMark: Towards Watermarking Neural Network Hardware},
  author={Clements, Joseph and Lao, Yingjie},
  journal={AAAI 2022},
  year={2022}
}

@inproceedings{matsumoto2022feasibility,
  title={A feasibility study of watermark embedding in RNN models},
  author={Matsumoto, Kota and Sakazawa, Shigeyuki},
  booktitle={International Workshop on Advanced Imaging Technology (IWAIT) 2022},
  volume={12177},
  pages={113--118},
  year={2022},
  organization={SPIE}
}

@inproceedings{jia2021robust,
  title={Robust and Verifiable Information Embedding Attacks to Deep Neural Networks via Error-Correcting Codes},
  author={Jia, Jinyuan and Wang, Binghui and Gong, Neil Zhenqiang},
  booktitle={Proceedings of the 2021 ACM Asia Conference on Computer and Communications Security},
  pages={2--13},
  year={2021}
}

@inproceedings{zhai2022adversarial,
  title={A Girl Has A Name, And It's... Adversarial Authorship Attribution for Deobfuscation},
  author={Zhai, Wanyue and Rusert, Jonathan and Shafiq, Zubair and Srinivasan, Padmini},
  booktitle={Proceedings of the 60th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)},
  pages={7372--7384},
  year={2022}
}

@article{ito2022access,
  title={Access Control of Semantic Segmentation Models Using Encrypted Feature Maps},
  author={Ito, Hiroki and MaungMaung, AprilPyone and Shiota, Sayaka and Kiya, Hitoshi},
  journal={arXiv preprint arXiv:2206.05422},
  year={2022}
}

@article{wang2022wet,
  title={Wet Paper Coding-Based Deep Neural Network Watermarking},
  author={Wang, Xuan and Lu, Yuliang and Yan, Xuehu and Yu, Long},
  journal={Sensors},
  volume={22},
  number={9},
  pages={3489},
  year={2022},
  publisher={MDPI}
}



@article{ito2021protecting,
  title={Protecting Semantic Segmentation Models by Using Block-wise Image Encryption with Secret Key from Unauthorized Access},
  author={Ito, Hiroki and AprilPyone, MaungMaung and Kiya, Hitoshi},
  journal={arXiv preprint arXiv:2107.09362},
  year={2021}
}

  

@article{yasui2022coded,
  title={Coded DNN Watermark: Robustness against Pruning Models Using Constant Weight Code},
  author={Yasui, Tatsuya and Tanaka, Takuro and Malik, Asad and Kuribayashi, Minoru},
  journal={Journal of Imaging},
  volume={8},
  number={6},
  pages={152},
  year={2022},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@inproceedings{li2020multi,
  title={The Multi-Watermarks Attack of DNN Watermarking},
  author={Li, Deyin and Yang, Yu},
  booktitle={2020 4th International Conference on Advances in Image Processing},
  pages={178--184},
  year={2020}
}

@article{rathi2021watermarking,
  title={Watermarking of Deep Recurrent Neural Network Using Adversarial Examples to Protect Intellectual Property},
  author={Rathi, Pulkit and Bhadauria, Saumya and Rathi, Sugandha},
  journal={Applied Artificial Intelligence},
  pages={1--18},
  year={2021},
  publisher={Taylor \& Francis}
}

@article{yan2022and,
  title={" And Then There Were None": Cracking White-box DNN Watermarks via Invariant Neuron Transforms},
  author={Yan, Yifan and Pan, Xudong and Wang, Yining and Zhang, Mi and Yang, Min},
  journal={arXiv preprint arXiv:2205.00199},
  year={2022}
}

@inproceedings{chen2022speech,
  title={Speech Pattern Based Black-Box Model Watermarking for Automatic Speech Recognition},
  author={Chen, Haozhe and Zhang, Weiming and Liu, Kunlin and Chen, Kejiang and Fang, Han and Yu, Nenghai},
  booktitle={ICASSP 2022-2022 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={3059--3063},
  year={2022},
  organization={IEEE}
}

@article{xu2021watermarking,
  title={Watermarking Graph Neural Networks based on Backdoor Attacks},
  author={Xu, Jing and Picek, Stjepan},
  journal={arXiv preprint arXiv:2110.11024},
  year={2021}
}

@inproceedings{huang2021novel,
  title={A Novel Watermarking Mechanism for Deep Learning Models based on Chaotic Boundaries},
  author={Huang, Zi-Jie and Zhang, Ying-Qian and Jia, Yi-Ran},
  booktitle={2021 15th International Symposium on Medical Information and Communication Technology (ISMICT)},
  pages={104--109},
  year={2021},
  organization={IEEE}
}

@article{sharma2022single,
  title={A single watermark based scheme for both protection and authentication of identities},
  author={Sharma, S and Zou, JJ and Fang, G},
  journal={IET Image Processing},
  year={2022},
  publisher={Wiley Online Library}
}

@article{tran2018spectral,
  title={Spectral signatures in backdoor attacks},
  author={Tran, Brandon and Li, Jerry and Madry, Aleksander},
  journal={Advances in neural information processing systems},
  volume={31},
  year={2018}
}

@inproceedings{gao2019strip,
  title={Strip: A defence against trojan attacks on deep neural networks},
  author={Gao, Yansong and Xu, Change and Wang, Derui and Chen, Shiping and Ranasinghe, Damith C and Nepal, Surya},
  booktitle={Proceedings of the 35th Annual Computer Security Applications Conference},
  pages={113--125},
  year={2019}
}

@inproceedings{black_wang2022ntl,
  title={Non-transferable learning: A new approach for model ownership verification and applicability authorization},
  author={Wang, Lixu and Xu, Shichao and Xu, Ruiqi and Wang, Xiao and Zhu, Qi},
  booktitle={International Conference on Learning Representations},
  year={2022}
}

@article{huang2022cmua,
  title={Cmua-watermark: A cross-model universal adversarial watermark for combating deepfakes},
  author={Huang, Hao and Wang, Yongtao and Chen, Zhaoyu and Li, Yuheng and Tang, Zhi and Chu, Wei and Chen, Jingdong and Lin, Weisi and Ma, Kai-Kuang},
  journal={AAAI},
  year={2022}
}

@inproceedings{white_li2022defending,
title={Defending against model stealing via verifying embedded external features},
author={Li, Yiming and Zhu, Linghui and Jia, Xiaojun and Jiang, Yong and Xia, Shu-Tao and Cao, Xiaochun},
year={2022},
organization={AAAI}
}

@inproceedings{sanyal2022towards,
  title={Towards Data-Free Model Stealing in a Hard Label Setting},
  author={Sanyal, Sunandini and Addepalli, Sravanti and Babu, R Venkatesh},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={15284--15293},
  year={2022}
}

@inproceedings{wang2022bppattack,
  title={BppAttack: Stealthy and Efficient Trojan Attacks against Deep Neural Networks via Image Quantization and Contrastive Adversarial Learning},
  author={Wang, Zhenting and Zhai, Juan and Ma, Shiqing},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={15074--15084},
  year={2022}
}

@inproceedings{sun2022coprotector,
  title={CoProtector: Protect Open-Source Code against Unauthorized Training Usage with Data Poisoning},
  author={Sun, Zhensu and Du, Xiaoning and Song, Fu and Ni, Mingze and Li, Li},
  booktitle={Proceedings of the ACM Web Conference 2022},
  pages={652--660},
  year={2022}
}

@inproceedings{sun2022coprotector,
  title={Model Stealing Defense against Exploiting Information Leak Through the Interpretation of Deep Neural Nets},
  author={Jeonghyun Lee, Sungmin Han, Sangkyun Lee},
  booktitle={JICAI},
  year={2022}
}

@inproceedings{zanella2021grey,
  title={Grey-box extraction of natural language models},
  author={Zanella-Beguelin, Santiago and Tople, Shruti and Paverd, Andrew and K{\"o}pf, Boris},
  booktitle={International Conference on Machine Learning},
  pages={12278--12286},
  year={2021},
  organization={PMLR}
}

@inproceedings{cun2021split,
  title={Split then refine: stacked attention-guided ResUNets for blind single image visible watermark removal},
  author={Cun, Xiaodong and Pun, Chi-Man},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={35},
  number={2},
  pages={1184--1192},
  year={2021}
}

@inproceedings{wang2021data,
  title={Data-free knowledge distillation with soft targeted transfer set synthesis},
  author={Wang, Zi},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={35},
  number={11},
  pages={10245--10253},
  year={2021}
}

@inproceedings{kang2021randomized,
  title={Randomized Generation of Adversary-Aware Fake Knowledge Graphs to Combat Intellectual Property Theft},
  author={Kang, Snow and Molinaro, Cristian and Pugliese, Andrea and Subrahmanian, VS},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={35},
  number={5},
  pages={4155--4163},
  year={2021}
}

@InProceedings{Mehra_2021_CVPR,
    author    = {Mehra, Akshay and Kailkhura, Bhavya and Chen, Pin-Yu and Hamm, Jihun},
    title     = {How Robust Are Randomized Smoothing Based Defenses to Data Poisoning?},
    booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
    month     = {June},
    year      = {2021},
    pages     = {13244-13253}
}
